RLE Plots: Visualising Unwanted Variation in High Dimensional Data

Unwanted variation can be highly problematic and so its detection is often crucial. Relative log expression (RLE) plots are a powerful tool for visualising such variation in high dimensional data. We provide a detailed examination of these plots, with the aid of examples and simulation, explaining what they are and what they can reveal. RLE plots are particularly useful for assessing whether a procedure aimed at removing unwanted variation, i.e. a normalisation procedure, has been successful. These plots, while originally devised for gene expression data from microarrays, can also be used to reveal unwanted variation in many other kinds of high dimensional data, where such variation can be problematic.

==> references <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Luke Gandolfo at 2017-01-30 13:27:26 +1100 


%% Saved with string encoding Unicode (UTF-8) 



@article{mandel1969,
	Author = {Mandel, John},
	Date-Added = {2017-01-30 02:26:40 +0000},
	Date-Modified = {2017-01-30 02:26:50 +0000},
	Journal = {Journal of Research of the National Bureau of Standards, Series B},
	Pages = {309--328},
	Title = {The partitioning of interaction in analysis of variance},
	Volume = {73},
	Year = {1969}}

@article{mandel1971,
	Author = {Mandel, John},
	Date-Added = {2017-01-30 02:26:10 +0000},
	Date-Modified = {2017-01-30 02:27:14 +0000},
	Journal = {Technometrics},
	Number = {1},
	Pages = {1--18},
	Publisher = {Taylor \&amp; Francis Group},
	Title = {A new analysis of variance model for non-additive data},
	Volume = {13},
	Year = {1971}}

@article{tukey1949,
	Author = {Tukey, John W},
	Date-Added = {2017-01-30 02:21:08 +0000},
	Date-Modified = {2017-01-30 02:21:18 +0000},
	Journal = {Biometrics},
	Number = {3},
	Pages = {232--242},
	Publisher = {JSTOR},
	Title = {One degree of freedom for non-additivity},
	Volume = {5},
	Year = {1949}}

@article{irizarry2003,
	Author = {Irizarry, Rafael A and Bolstad, Benjamin M and Collin, Francois and Cope, Leslie M and Hobbs, Bridget and Speed, Terence P},
	Date-Added = {2017-01-19 05:36:30 +0000},
	Date-Modified = {2017-01-19 05:37:47 +0000},
	Journal = {Nucleic acids research},
	Number = {4},
	Pages = {e15},
	Publisher = {Oxford Univ Press},
	Title = {Summaries of {A}ffymetrix {G}ene{C}hip probe level data},
	Volume = {31},
	Year = {2003}}

@article{vawter2004,
	Author = {Vawter, Marquis P and Evans, Simon and Choudary, Prabhakara and Tomita, Hiroaki and Meador-Woodruff, Jim and Molnar, Margherita and Li, Jun and Lopez, Juan F and Myers, Rick and Cox, David and others},
	Date-Added = {2017-01-19 00:20:23 +0000},
	Date-Modified = {2017-01-19 00:20:47 +0000},
	Journal = {Neuropsychopharmacology},
	Number = {2},
	Pages = {373},
	Publisher = {NIH Public Access},
	Title = {Gender-specific gene expression in post-mortem human brain: localization to sex chromosomes},
	Volume = {29},
	Year = {2004}}

@article{risso2014,
	Author = {Risso, Davide and Ngai, John and Speed, Terence P and Dudoit, Sandrine},
	Date-Added = {2016-12-22 05:58:13 +0000},
	Date-Modified = {2016-12-22 05:59:13 +0000},
	Journal = {Nature biotechnology},
	Number = {9},
	Pages = {896--902},
	Title = {Normalization of {RNA}-seq data using factor analysis of control genes or samples},
	Volume = {32},
	Year = {2014}}

@book{scherer2009,
	Author = {Scherer, Andreas},
	Date-Added = {2016-12-21 06:05:53 +0000},
	Date-Modified = {2016-12-21 06:06:15 +0000},
	Publisher = {John Wiley \& Sons},
	Title = {Batch effects and noise in microarray experiments: sources and solutions},
	Year = {2009}}

@article{gagnon2012,
	Author = {Gagnon-Bartsch, Johann A and Speed, Terence P},
	Date-Added = {2016-09-07 05:25:48 +0000},
	Date-Modified = {2016-09-07 05:31:30 +0000},
	Journal = {Biostatistics},
	Number = {3},
	Pages = {539--552},
	Publisher = {Biometrika Trust},
	Title = {Using control genes to correct for unwanted variation in microarray data},
	Volume = {13},
	Year = {2012}}

@article{brettschneider2008,
	Author = {Brettschneider, Julia and Collin, Fran{\c{c}}ois and Bolstad, Benjamin M and Speed, Terence P},
	Date-Added = {2016-09-07 05:25:00 +0000},
	Date-Modified = {2016-09-08 04:39:33 +0000},
	Journal = {Technometrics},
	Number = {3},
	Pages = {241--264},
	Publisher = {Taylor \&amp; Francis},
	Title = {Quality assessment for short oligonucleotide microarray data},
	Volume = {50},
	Year = {2008}}

@incollection{bolstad2005,
	Author = {Bolstad, BM and Collin, F and Brettschneider, J and Simpson, K and Cope, L and Irizarry, RA and Speed, TP},
	Booktitle = {Bioinformatics and computational biology solutions using R and bioconductor},
	Date-Added = {2016-09-07 05:23:38 +0000},
	Date-Modified = {2016-09-07 05:31:15 +0000},
	Pages = {33--47},
	Publisher = {Springer},
	Title = {Quality assessment of Affymetrix GeneChip data},
	Year = {2005}}

